Prompt-based Code Completion via Multi-Retrieval Augmented Generation

Automated code completion, aiming at generating subsequent tokens from unfinished code, has been significantly benefited from recent progress in pre-trained Large Language Models (LLMs). However, these models often suffer from coherence issues and hallucinations when dealing with complex code logic or extrapolating beyond their training data. Existing Retrieval Augmented Generation (RAG) techniques partially address these issues by retrieving relevant code with a separate encoding model where the retrieved snippet serves as contextual reference for code completion. However, their retrieval scope is subject to a singular perspective defined by the encoding model, which largely overlooks the complexity and diversity inherent in code semantics. To address this limitation, we propose ProCC, a code completion framework leveraging prompt engineering and the contextual multi-armed bandits algorithm to flexibly incorporate and adapt to multiple perspectives of code. ProCC first employs a prompt-based multi-retriever system which crafts prompt templates to elicit LLM knowledge to understand code semantics with multiple retrieval perspectives. Then, it adopts the adaptive retrieval selection algorithm to incorporate code similarity into the decision-making process to determine the most suitable retrieval perspective for the LLM to complete the code. Experimental results demonstrate that ProCC outperforms state-of-the-art code completion technique by 8.6% on our collected open-source benchmark suite and 10.1% on the private-domain benchmark suite collected from a billion-user e-commerce company in terms of Exact Match. ProCC also allows augmenting fine-tuned techniques in a plug-and-play manner, yielding 5.6% improvement over our studied fine-tuned model.

==> algorithms/linUCB.tex <==
\SetKwInput{KwInput}{Input} % Set the Input
\SetKwInput{KwOutput}{Output} % set the Output
\SetAlCapFnt{\footnotesize}
\SetKwComment{Comment}{$\triangleright$\ }{}
\SetCommentSty{mycommfont}
\DontPrintSemicolon

\begin{algorithm}[th]
\footnotesize
\setstretch{1.1}
\caption{\footnotesize Adaptive Retrieval Selection}
\label{alg:linucb}

\SetKwFunction{FTrain}{TrainLinUCB}
\SetKwFunction{FInfer}{SelectRetrieval}
\SetKwProg{Fn}{Function}{:}{}
\KwInput{\( \alpha \in \mathbb{R}_+, \text{num\_arms}, d \in \mathbb{N}, \text{validation set } \mathcal{V}, \text{test set } \mathcal{T} \)}
\KwOutput{Trained parameters \( A, b \) and chosen retrieval for test set}

\Fn{\FTrain{\(\alpha, \text{num\_arms}, d, \mathcal{V}\)}}{
    \( A \leftarrow I_d \) \Comment*[r]{Identity matrix for each arm}
    \( b \leftarrow 0_d \) \Comment*[r]{Reward vector for each arm}
    \For{\( t \) in \( \mathcal{V} \)}{
        \( \theta_t \leftarrow A^{-1}b \) \\
        \For{\( a = 1 \) \KwTo \( \text{num\_arms} \)}{
            Observe features \( x_{t,a} \) including cosine and Jaccard similarities \\
            \( p_{t,a} \leftarrow \theta_t^\top x_{t,a} + \alpha \sqrt{x_{t,a}^\top A^{-1}x_{t,a}} \) \\
        }
        \( a_t \leftarrow \arg\max_a p_{t,a} \) \\
        \( r_t \leftarrow 0 \) \Comment*[r]{Initialize reward to 0}
        \If{action \( a_t \) is an exact match}{
            \( r_t \leftarrow 1 \) \Comment*[r]{Set reward to 1 for exact match}
        }
        \( A \leftarrow A + x_{t,a_t}x_{t,a_t}^\top \) \\
        \( b \leftarrow b + x_{t,a_t}r_t \) \\
    }
    \Return \( A, b \) \\
}

\Fn{\FInfer{\(A, b, t\)}}{
    \( \theta_t \leftarrow A^{-1}b \) \\
    \For{\( a = 1 \) \KwTo \( \text{num\_arms} \)}{
        Observe features \( x_{t,a} \) including cosine and Jaccard similarities \\
        \( p_{t,a} \leftarrow \theta_t^\top x_{t,a} \) \\
    }
    \( a_t \leftarrow \arg\max_a p_{t,a} \) \\
    \Return \( a_t \) \\
}

% \( A, b \leftarrow \) \FTrain{\(\alpha, \text{num\_arms}, d, \mathcal{V}\)} \\
% \For{\( t \) in \( \mathcal{T} \)}{
%     \( a_t \leftarrow \) \FInfer{\(A, b, t\)} \\
%     \Comment*[r]{Execute chosen action and observe result (optional)}
% }
\end{algorithm}


==> algorithms/retrieval.tex <==
% 这里是Faiss Retrieval的实验结果，已经完成了入库切块等操作，使用Query Code查询top-k相似的代码片段，不太对，需要突出RAG-Fusion，我们的核心路数还是RAG-Fusion。
% 这里要改成RAG-Fusion, 这个算法表会长一倍。
\SetKwFor{While}{while}{do}{}
\SetKwInput{KwInput}{Input}
\SetKwInput{KwResult}{Result}
\SetKw{KwReturn}{return}
\SetAlCapFnt{\footnotesize}
\SetKwComment{Comment}{$\triangleright$\ }{}
\SetCommentSty{mycommfont}
\DontPrintSemicolon
\begin{algorithm}[t]
\footnotesize
\setstretch{1.1}
\caption{\footnotesize Retrieval top-k similar code snippets}
\label{alg:link-locality}
    \KwInput{\textit{query\_code, FaissDB} \Comment*[r]{Code blocks}}
    \KwResult{\textit{top\_k similar code snippets} \Comment*[r]{Similar Codes}}
    
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{QueryTopK} {
        \textit{results} $\leftarrow$ $\emptyset$ \\
        \textit{top-k} $\leftarrow$ \textit{faissdb.search\_with\_score(query\_code)} \\
        \For{(\textit{doc}, \textit{score}) $\in$ \textit{top-k}} {
            \textit{result.add(code:doc.page\_context, distance: score)} \\
            
        }
        \textit{result.sort(key=lambda x : x['distance']} \\
        \KwRet \textit{results}
    }
    \;
    \SetKwProg{Fn}{Function}{:}{}
    \Fn{ReSort(top-k)} {
        \textit{resort\_results} $\leftarrow$ $\emptyset$ \\
        \For{\textit{snippets} $\in$ \textit{top-k}} {
            \textit{score} $\leftarrow$ \textit{JaccardSimilarity(query\_code, snippet.code)} \\
            \textit{result.add(code:snippet.code, score: score)} \\
        }
        \textit{resort\_result.sort(key=lambda x : x['score']} \\
        \KwRet \textit{resort\_results}
    }
\end{algorithm}


==> sections/approach/0_approach.tex <==
\section{Approach}
% 改为写RAG，这部分的workflow只是提到的一个点，应该在文章以开头就应该提出RAG来强调我们的工作。
% \begin{figure*}[ht]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figures/workflow.pdf}
%   \caption{The workflow of \method{} \ql{Numbers represent importance}}
%   \label{fig:workflow}
% \end{figure*}

\input{sections/approach/1_task}
% 大模型微调 1， 应该删除这部分，直接讲RAG。 故事线还是不够清晰。
\input{sections/approach/2_fine_tune}
% RAG 5
\input{sections/approach/3_rag}
% RAG+SFT 2
\input{sections/approach/4_rag_sft}
% 开发者反馈 2
\input{sections/approach/5_feedback}


==> sections/approach/1_task.tex <==
\subsection{Task Description}
% 要修改下面的repo描述，改为domain，这里要修改描述。

Given a large pre-trained language model $\mathcal{M}$, the task of automated code completion can be formulated as predicting the token sequence $\hat{Y} = \mathcal{M}(\hat{X})$, where $\hat{X}$ denotes the unfinished in-file code snippet comprising the prefix before and suffix after the cursor position, as exemplified in list 1, we use a \texttt{Fill\_Me} token to indicate the position need to predict.

To augment the language model $\mathcal{M}$ with relevant contextual information, we introduce a code retrieval model $\mathcal{R}$ and construct a Retrieval-Augmented Generation (RAG) framework. Specifically, we split the codebase into code snippets $C= \{c_1, c_2, ...\}$. For an unfinished snippet $\hat{X}$, we apply $\mathcal{R}$ to retrieve the most relevant snippets $C_{ret} = \mathcal{R}(C, \hat{X})$ from the repository. Subsequently, code completion is performed by using $\mathcal{M}$ to generate the predicted token sequence based on the retrieved snippets, i.e., $\hat{Y} = \mathcal{M}(C_{ret}, \hat{X})$. The key advantage of this RAG approach is that it allows incorporating useful contextual signals from the code codebase during completion, enhancing the modeling capacity of $\mathcal{M}$.

%use pdf? ppt->write code->pdf
\begin{lstlisting}[language=Java, caption=Fill in Middle Example]
public class FenwickTree {
    private int[] tree;
    private int size;

    public FenwickTree(int n) {
        this.size = n;
        this.tree = new int[n + 1];
    }

    public void update(int index, int value) {
        [Fill_ME]
    }

    public int query(int index) {
        int result = 0;
        while (index > 0) {
            result = Math.max(result, this.tree[index]);
            index -= index & -index;
        }
        return result;
    }
}
\end{lstlisting}

==> sections/approach/2_fine_tune.tex <==
\subsection{Fine Tuning}
In alignment with contemporary research in large code models~\cite{instructgpt}, we adopt a two-stage training strategy, consisting of incremental learning and Supervised Fine-tuning (SFT). The incremental learning phase utilizes the fill-in-middle (FIM) format, allocating training data across various formats to enhance the model's proficiency in handling extensive contextual information. This setup prepares the model to adeptly generate tokens in code completion scenarios by integrating both preceding and succeeding contexts.

Supervised Fine-tuning shifts to a supervised learning approach. Utilizing the tree-sitter\footnote{\url{https://tree-sitter.github.io/tree-sitter/}} AST analysis tool, the SFT phase concentrates on extracting code blocks to form the SFT dataset. Unlike the pretraining phase, where loss computation is widespread across each token, the SFT phase specifically targets the output section for loss calculation. This targeted approach in SFT fine-tunes the model's capability to produce accurate and relevant code completions.

The SFT dataset, constructed around functions and code blocks, serves as a benchmark for the model's efficiency in suggesting contextually appropriate code continuations, thus fostering effective software development.


==> sections/approach/3_rag.tex <==
\subsection{RAG}
\begin{figure}[h]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/rag_flow.pdf}
  \caption{RAG Flow}
  \label{fig:rag_flow}
\end{figure}
As shown in figure~\ref{fig:rag_flow}, retrieval-augmented generation (RAG) stands as a pivotal enhancement for generative large language models, significantly boosting their accuracy and reliability by incorporating facts fetched from external sources. This innovative approach fills a crucial gap in the operational mechanics of Large Language Models (LLMs). While LLMs inherently encapsulate a deep understanding, or parameterized knowledge, of human language patterns, their capabilities are sometimes limited in addressing more specific or current topics. RAG addresses this limitation by providing models with citable sources, akin to research paper footnotes, thereby fostering user trust and reducing potential inaccuracies in responses, a phenomenon often referred to as hallucination.

Furthermore, RAG offers a cost-effective and efficient alternative to retraining models with additional datasets. It allows for the dynamic incorporation of new information sources, thus facilitating a more adaptable and responsive LLM system. The essence of RAG lies in its ability to facilitate interactions between users and data repositories, heralding new kinds of user experiences. This versatility underscores the vast potential applications of RAG, extending far beyond the scope of available datasets.

The following subsections, 'Dense Retrieval' and 'Sparse Retriever', delve into the specific implementations of RAG in the context of code completion. These sections exemplify how RAG enhances the retrieval of relevant code snippets, leveraging both deep semantic understanding and efficient lexical similarity measures.

\paragraph{Embedding-based Similar Code Retrieval}
Embedding-based Similar Code Retrieval is an approach centered around the utilization of code embeddings for the retrieval of similar code snippets. Initially, code snippets are transformed into fixed-length vector representations, known as code embeddings. This is typically achieved through the parsing of the code's abstract syntax tree, supplemented by the employment of models such as Recurrent Neural Networks (RNNs) and Transformers, which are instrumental in deriving the embedding expressions.

Following this, an extensive code corpus is compiled, with embeddings extracted for each code snippet within it. When a new code query is introduced, it undergoes a similar process of embedding generation. The core of the retrieval process involves identifying the top-K most similar code snippets from the corpus. This identification hinges on finding snippets whose embeddings most closely align with those of the query.

Moreover, the quantification of similarity between code snippets is computed through the cosine similarity of their embedding vectors. Cosine similarity, in this context, serves as a metric for the degree of similarity, by evaluating the cosine of the angle between the embedding vectors of the code snippets in question. This method effectively capitalizes on the embedded semantic characteristics of the code, thereby enabling a more nuanced and precise retrieval based on code similarity.

\paragraph{Sparse retriever}
The sparse retriever utilized in our framework is based on BM25, leveraging the robust implementation provided by ElasticSearch\footnote{\url{https://www.elastic.co/elasticsearch}}. BM25, a term-based retrieval method, treats each code fragment as a sequence of code tokens and employs a bag-of-words model to represent these sequences. This model focuses on the frequency of terms within the documents, disregarding their order, thus enabling a straightforward yet effective mechanism for capturing lexical similarities. The BM25 score, calculated between a query and a document, quantifies this similarity, with higher scores indicating greater lexical correspondence. This mechanism is particularly effective in identifying relevant code fragments that share a significant number of common terms with the query, thereby facilitating efficient retrieval of pertinent code segments in a vast corpus.

Meanwhile, the integration of the Jaccard similarity measure further refines our sparse retrieval strategy. This measure, grounded in set theory, is quantitatively defined as \(\text{Jaccard}(A, B) = \frac{|A \cap B|}{|A \cup B|}\), where \(A\) and \(B\) represent the sets of tokens in the query and the document, respectively. By calculating the proportion of shared tokens, the Jaccard similarity provides an additional dimension to evaluate the overlap between query and document. This approach, in tandem with BM25, enriches the retrieval process by offering a dual-perspective assessment of similarity, thus enhancing the system's capability to accurately identify relevant code fragments within an extensive corpus.

\subsection{RAG-Fusion}
We use different prompt to embedding the code snippets.

\paragraph{RAG-Fusion in Code Completion}
The RAG-Fusion approach represents an advanced stage in the evolution of code completion methodologies. This section delves into how different components of the RAG framework are fused to enhance the performance of code completion models.

\paragraph{Integrating Multiple RAG Components:} RAG-Fusion involves the strategic amalgamation of multiple RAG elements such as block, function, class, and real-time information. This fusion aims to leverage the unique strengths of each component, thereby creating a more robust and versatile code completion tool.

\paragraph{Benefits of RAG-Fusion:} The primary advantage of RAG-Fusion lies in its ability to enhance model performance by incorporating a broader range of contextual signals from the codebase. This is particularly beneficial in scenarios where conventional RAG approaches might fall short due to limited context or overly specific retrieval results.

\subsection{Integration of RAG Strategies using LinUCB Algorithm}
In our approach, we employ the LinUCB algorithm to effectively integrate various Retrieval-Augmented Generation (RAG) strategies. LinUCB, a contextual bandit algorithm, is adept at balancing the exploration and exploitation trade-off. By using LinUCB, we dynamically adjust the weight given to different RAG strategies based on their performance in real-time scenarios. This method allows the model to adaptively learn which RAG strategies are most effective in various contexts of code completion. The adaptive nature of LinUCB ensures that our system continuously evolves, fine-tuning its retrieval strategies to optimize code completion accuracy and relevance.
\input{algorithms/linUCB}

\subsubsection{hypothetical line embedding}

% \input{algorithms/retrieval}

% % 召回AST最相似的代码文件？
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.9\linewidth]{figures/rag_fusion.pdf}
%   \caption{RAG Fusion Flow}
%   \label{fig:rag_fusion}
% \end{figure}


\subsection{Prompt Based Embedding}
Use different prompts to retrieve information of different semantic information.

==> sections/approach/4_rag_sft.tex <==
\subsection{RAG-based SFT}
% 基于我们之前的分析，RAG在增强大模型代码补全能力方面有很不错的表现。但是RAG只工作在推理截断，RAG的召回的信息并没有进一步用来训练大模型。基于该动机，我们提出一个关键问题，将RAG集成到训练阶段能在多大程度上提升模型的整体性能。在现实世界的编码应用中，我们发现每个代码文件的token数一般都比较少，具体的，我们统计了公司内部的将近100w个代码文件，并计算了其平均token数目，结果发现平均每个代码文件只包含了1195.82个token，大约100行的代码，这一数字远远低于现在常规LLMs的训练样本长度预置（比如，Code llama的训练长度为4096，并进一步做了LCFT，长度为16k）这一观察结果凸显了传统训练过程中的一个关键挑战：简单地串联不同的样本信息来人为地延长样本长度是一种次优做法，因为它无法有效地利用模型处理和解释长程上下文信息的能力。基于此我们首次提出通过RAG的信息扩充原样本的长度，以进一步释放大模型的能力。
Based on our previous analysis, RAG demonstrates notable performance in enhancing the code completion capabilities of large models. However, RAG only operates at the inference truncation, and the information recalled by RAG is not further utilized to train the large models. Motivated by this, we pose a critical question: to what extent can integrating RAG into the training phase boost the overall performance of the model? In real-world coding applications, we find that each code file typically contains a relatively small number of tokens. Specifically, we analyzed nearly 1 million code files within our company and calculated their average token count. The results revealed that each code file contains an average of only 1195.82 tokens, approximately 100 lines of code, a figure significantly lower than the preset training sample length of conventional LLMs (for example, \codellama{} training length is 4096, further extended to 16k through long context fine tune). This observation highlights a key challenge in the traditional training process: simply concatenating different sample information to artificially extend the sample length is a suboptimal approach, as it fails to effectively leverage the model's ability to process and interpret long-range contextual information. Based on this, we propose for the first time to augment the original sample length with information from RAG, further unleashing the potential of large models.

% 这里讲具体的做法
% 特别的，原始模型的训练样本格式为sample = "PRE" + prefix + "SUF" + suffix + "MID" + output，我们通过RAG召回相似的信息并将这些额外的补充信息添加到prefix之前，sample = "PRE" + RAG + prefix + "SUF" + suffix + "MID" + output，在4k的训练长度预算下，我们分配1024个token给RAG部分信息，尽可能保留原文件的信息比例。这进一步丰富了模型的信息提取能力，进一步提升模型的推理能力。
\begin{figure}[h]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/rag_sft.pdf}
  \caption{RAG Flow}
  \label{fig:rag_sft}
\end{figure}

A significant modification has been made to the training sample format of the original model, enhancing its capacity for contextual understanding. The original format:
\begin{align*}
    \text{sample} &= \texttt{"PRE"} + \text{prefix} + \texttt{"SUF"} + \text{suffix} + \texttt{"MID"} + \text{output}
\end{align*}
has been restructured with the integration of RAG-retrieved information, placed strategically before the prefix:
\begin{align*}
    \text{sample} &= \texttt{"PRE"} + \text{RAG} + \text{prefix} + \texttt{"SUF"} + \text{suffix} + \texttt{"MID"} + \text{output}
\end{align*}
This enhancement, under a 4k token training length budget, allocates 1024 tokens to the RAG component, ensuring the preservation of the original file's informational proportionality. This strategic allocation broadens the model's ability for information extraction and augments its inferential capabilities, proving crucial in complex code completion tasks.

% 这才是真正的Context Rich, 是否也可以讲一下快手最初的做法，简单的加一个Path, Language也能提升效果？
% 通过这种RAG增强的训练样本方法，我们显著地提升了模型对复杂编码环境的理解和适应能力。这一方法不仅克服了传统训练样本格式的局限性，而且为模型提供了更为丰富和多样化的上下文信息。特别地，RAG部分的引入增强了模型在长程上下文处理和解释方面的能力，这对于提高代码补全任务中的准确性和效率至关重要。总的来说，这一创新性的训练策略为模型提供了更深入的代码理解，从而弥补了之前的训练缺陷，并为实现高效且精确的代码补全设定了新的标准。

This enhanced training methodology, enriched by RAG-augmented training samples, significantly elevates the model’s comprehension and adaptability within complex coding environments. By transcending the limitations of traditional training sample formats, this approach provides the model with a richer and more varied contextual backdrop. The inclusion of the RAG component notably bolsters the model's capacity to process and interpret extended contexts, an aspect crucial for enhancing accuracy and efficiency in code completion tasks. In essence, this innovative training strategy endows the model with a deeper understanding of code, effectively addressing previous training deficiencies and setting new benchmarks for efficient and precise code completion.

==> sections/approach/5_feedback.tex <==
\subsection{Developers FeedBack}
% 但是这里要说明是如何起作用的？更新测试集？修改SFT数据？感觉这个section太工程化，是否考虑删除呢？
% 这部分直接独立成RQ3，RQ3主讲工程实践部分。
Our analysis indicated that while the open-source model excels in generalization, it falters when catering to specific requirements. To enhance the model's targeted performance, we conducted a questionnaire-based study, garnering feedback from 152 real developers. The majority of developers favored predictions concerning the content of the current and ensuing lines, along with API suggestions. Informed by these authentic developer insights, we aim to refine our Supervised Fine-tuning (SFT) dataset construction approach to augment the accuracy of model continuations.


==> sections/evaluation/3_result_and_analysis.tex <==
\subsection{Results and Anslysis}
% 这一整个部分都需要重写。
\subsubsection{RQ1}
As shown in~\ref{tab:main_results}, \ourmethod{} exhibits the most substantial improvement compared with baselines.

The data presented in Table~\ref{tab:rq2} suggests that state-of-the-art (SOTA) in-context learning techniques such as Retrieval-Augmented Generation (RAG) significantly enhance code completion results. The performance metrics, namely ACC and BLEU, show improvement in transitioning from OS to OS+RAG. Furthermore, RAG-Fusion, an extended approach, yields further improvement, indicating that integrating RAG with fusion techniques amplifies the benefits, as evidenced by the increase in ACC and BLEU scores, and the decrease in Edit-distance from OS+RAG to OS+RAG+Fusion. Therefore, RQ2 is affirmatively answered; both RAG and RAG-Fusion contribute to enhanced code completion outcomes. Suggesting that if presented only at inference time, similar contexts help code completion more.

\begin{figure}[ht]
  \centering
  \includegraphics[width=0.9\linewidth]{figures/Venn_4.png}
  \caption{prompt venn}
  \label{fig:prompt_venn}
\end{figure}

\input{tables/rq2}

\subsubsection{RQ3}
To address RQ3, we conducted a questionnaire survey within real-world development scenarios, collecting 152 genuine user feedback entries. The feedback affirmed the effectiveness of our tool, and moving forward, we plan to refine our model based on the insights provided by the developers. This iterative refinement aims to tailor the model to better meet developers' requirements and enhance its performance in real-world deployments.

\begin{figure}[h]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/feedback.pdf}
  \caption{Developers Feedback}
  \label{fig:feedback}
\end{figure}


% 这里可能会涉及到为什么不同类型的测试集表现不同。
% One possible reason is that general code completion on average involves easier prediction locations such as boiler-plate code and code idioms.

==> sections/evaluation/4_ablation_study.tex <==
\subsection{Ablation Study}
% ablation study应该融合进RQ里面，到时候看看怎么合并进去。
\paragraph{Different RAG Configurations}
% 不同的RAG召回策略有什么效果，这个目前已有了初步的结果，fusion正在做。
In our ablation study, we explore the contributions of various RAG contents to the outcomes by assessing the impact of different RAG contents on the results, encompassing block, function, class, PromptBert, and real-time information, among others. Additionally, we introduce a comparison with a randomly generated RAG (Random RAG) to serve as a baseline for our evaluation. This comparison is pivotal as it helps to delineate the efficacy of our selected RAG contents by providing a reference point for improvement over a random baseline. Our findings suggest that a fusion of these elements yields the most favorable results, with real-time information making a significant contribution. The comparison with Random RAG further underscores the effectiveness of our chosen RAG configurations in enhancing code completion outcomes.
\input{tables/ab1}

\paragraph{Top-k}
% 这个应该是在最好的结果的基础上，进一步验证性能，而不是直接去写。
% 在本章节，我们研究了top-k对生成结果的影响，由于长度的限制。
In previous results, we concatenated the top-1 retrieval snippet into the prompt to help the model in generating. In this section, we explore the performance implications of integrating multiple retrieval results.
% 结果分析
\input{tables/ab2}

\paragraph{Length}
The result of different prompt lengths with more RAG information.
\input{tables/ab3}

\paragraph{Compare with RAG-SFT}
\paragraph{Training Dataset}
In the pretraining phase, we significantly augment our training dataset with an additional 1 billion tokens, thereby enriching the exposure of \codellama{} to domain-specific code distributions—a notable enhancement over the open-source models. Subsequently, in the Supervised Fine-tuning phase, we further expand the training regimen by incorporating an extra 2 billion tokens. This robust data infusion across both phases aims to substantially bolster the model's understanding and performance in code completion tasks, aligning it more closely with real-world programming paradigms in both \python{} and \java{} languages.

\paragraph{Training Setup}
In alignment with the configuration delineated in \codellama{}~\cite{roziere2023codellama}, we adopt a learning rate of \(2 \times 10^{-5}\) coupled with a cosine schedule. The optimization is carried out using the AdamW optimizer~\cite{loshchilov2017decoupledadamw}. During the fine-tuning stage, Code Llama is trained on an NVIDIA A100 cluster, employing the DeepSpeed framework~\cite{rajbhandari2020zero} to enhance training efficiency and scalability. This setup is meticulously selected to harmonize with the extensive training data, ensuring a conducive environment for the model to effectively learn and adapt across the diverse code completion tasks.
% 这里就用图了，不用表格了。


\input{tables/ab4}
% 这里搞一张图就行，证明RAG对于SFT之后的模型同样有效。 这里进一步说明我们拿RAG去SFT，其实RAG sft也能写一篇paper，增强内容的关联度嘛。 不过感觉比较偏AI？


% Compare with GitHub copilot.
% 我们让实习生实际使用Copilot对比，Kwaipilot实际生成效果要比Copilot好，在私域的一些API上，但是在一些比较通用的补全任务上，Copilot要略好一些。这里补一个veen图。
\paragraph{Comparison with Copilot}
We engaged interns to utilize Copilot for a comparative analysis. Our results indicate that \method{} generates superior results compared to Copilot for certain APIs within the private domain. However, Copilot exhibits a slight advantage in performing more generalized code completion tasks.


\begin{figure}[h]
  \centering
  \includegraphics[width=0.98\linewidth]{figures/venn.pdf}
  \caption{Compare with Copilot}
  \label{fig:compare_with_copilot}
\end{figure}


% 注意因为CodeGen等模型不支持FIM格式，因此我们只给这些模型前缀部分信息，但是这样处理模型往往不知道在哪里停止，因此我们在模型写完当前block块停止输出。为了公平对比，我们对FIM的模型也做了同样的处理操作。只取输出的当前block块的信息，而不是应用所有的。

==> sections/old2_background.tex <==
\section{Background}
% 介绍三部分
% 1. 代码大模型
% 2. 代码补全任务
% 3. RAG？这里还需要考虑一下

\subsection{LLMs for Code}
The recent advancements in Natural Language Processing (NLP) have significantly catalyzed the evolution of large language models, thus transforming the landscape of code completion. Broadly speaking, these models can be categorized into open-source and proprietary (closed-source) models~\cite{zan2023large}.

On the one hand, open-source models such as CodeGen~\cite{nijkamp2023codegen}, StarCoder~\cite{starcoder}, and Code Llama~\cite{roziere2023codellama} have made significant strides. Firstly, CodeGen emerges as a tailored solution for code generation, providing a multi-turn program synthesis benchmark named Multi-Turn Programming Benchmark (MTPB) for nuanced evaluation and ascertaining program synthesis performance through iterative dialogues~\cite{nijkamp2023codegen}. Subsequently, StarCoder, a collaborative endeavor between Hugging Face~\cite{huggingface} and ServiceNow, encapsulates over 80 programming languages, addressing salient challenges in code generation including correctness, robustness, and safety. It improves quality and performance metrics compared to previous models such as PaLM~\cite{chowdhery2023palm}, LLaMA~\cite{touvron2023llama}, and OpenAI code-cushman-001~\cite{starcoder}. Recently, Code Llama, built atop Llama 2, excels in generating code and natural language elucidations about code, offering stable generations extending up to 100,000 tokens, significantly aiding in debugging and code completion within expansive codebases. It provides three model sizes: 7B, 13B, and 34B parameters, for different use cases including code completion, debugging, and generating functions based on prompts~\cite{roziere2023codellama}.

On the other hand, proprietary models such as GPT-4~\cite{openai2023gpt4} and Claude2~\cite{claude2} have also exhibited remarkable capabilities in code completion. However, they entail certain limitations. The closed-source nature of these models hinders their migration across different domains. Furthermore, the high costs associated with accessing or utilizing these proprietary models can be prohibitive, thereby limiting their adoption and adaptability across varying contexts.

Despite the exceptional code generation capability exhibited by these models, certain persistent issues such as hallucination phenomena and the inability to produce high-quality code remain unaddressed, across both open-source and proprietary models. This situation underscores the necessity of continued research, exploration, and refinement in this domain to unlock more reliable and cost-effective solutions for code completion.


\subsection{Code Completion}
% 代码补全，传统的技术代码补全主要是基于规则的，对长串的代码补全无法很好的处理。
Code completion is a prevalent feature in modern Integrated Development Environments (IDEs), serving as an interactive tool during a programmer's developmental activities. It provides constructive suggestions based on the current editing context, which includes identifiers, and interface calls, among others, significantly reducing the complexity of software development~\cite{github-copilot-2023, tabnine, lsp, jetbrains, vscode}. Traditional code completion methods largely rely on rule-based strategies. For instance, the code completion feature in JetBrains IDEs~\cite{jetbrains} excels at handling routine tasks. However, its ability to manage extensive code sequences or nuanced code structures may be limited due to the underlying rule-based mechanisms. While these conventional approaches can achieve high accuracy, their potential for enhancement is relatively limited, especially in extending long code strings.

% 指出开源代码大模型的问题，主要是三方面1.数据缺失，没有训练过。2. Context内容有限，只局限于当前文件。3. 长度有限，目前模型训练是4k长度，只能处理有限的信息
Recent advancements in Large Language Models (LLMs) showcase their potential to generate verbose and complex programs. However, there are limitations concerning the size of the code context and the lack of relevant training data, which may lead LLMs to perceive programs simplistically as mere sequences. This simplistic perception compromises their program analysis capability, consequently generating unreasonable code~\cite{chen2021evaluating, codet5+, nijkamp2023codegen}.

% 我们结合训练与RAG，解决上面提出的三个问题。
In this paper, we introduce a methodology for augmenting large models with supplementary information to guide them towards generating more accurate results. This effort aims to address the existing shortcomings and enhance the robustness of code completion systems, surpassing the limitations of traditional rule-based approaches. The potential integration of Large Language Models (LLMs) within Integrated Development Environments (IDEs) like JetBrains could open new avenues in code completion, making the coding process more intuitive and less burdensome for developers.


\subsection{RAG}
% 感觉这里需要重写
% 主要介绍了ReACC
The Retrieval-Augmented Generation (RAG) technology, an AI framework designed to enhance the quality of responses generated by Large Language Models (LLMs) by grounding them on external sources of knowledge, has been employed in the realm of code completion to bolster both the efficacy and efficiency of software development~\cite{meta2020rag}. A prime exemplification of this application is encapsulated in the ReACC framework~\cite{lu2022reacc}. Unlike conventional methodologies that predominantly zero in on the internal context within a file or project, ReACC innovatively incorporates "external" context, simulating the human propensity of referencing correlative code snippets during coding endeavors. This framework, proposed by Lu et al., accentuates the augmentation of code completion by harnessing both internal and external code contexts, leveraging a two-stage approach that combines a source code retriever and an auto-regressive language model. 

Central to ReACC are two components: firstly, a dual-encoder model acting as a code-to-code search retriever, tasked with fetching semantically and lexically akin code snippets from an extensive codebase; secondly, an auto-regressive language model, designated as the code completion generator, poised to predict ensuing code tokens predicated on the amalgamated context of the unfinished code and the retrieved code snippets. Through its innovative framework, ReACC has manifested exemplary performance on the CodeXGLUE benchmark across Python and Java programming languages, albeit its validation has been chiefly on smaller models, thereby indicating a scope of exploration regarding its scalability and performance on LLMs.

% 这里可以不要。
\subsection{Motivation}
In recent years, open-source Large Language Models (LLMs) have exhibited remarkable performance in code generation tasks, achieving results that are inspiring. However, a notable limitation of these LLMs is their training on open-source code, which impinges on their ability to effectively understand and generate code for private domain data, such as specific sub-libraries and APIs. To address this, we propose a comprehensive scheme to migrate open-source LLMs to private domain codes and conduct a thorough evaluation of their performance post-migration. Through evaluations on an internal test set, we observed a significant improvement in exact matching accuracy by 97.88\% and CodeBLEU score by 59.63\%.



Automated code completion, aimed at generating subsequent tokens from unfinished code, has been significantly benefited from recent progress in pre-trained Large Language Models (LLMs). However, these models often suffer from coherence issues and hallucinations when dealing with complex code logic or extrapolating beyond their training data. Existing Retrieval Augmented Generation (RAG) techniques partially address these issues by retrieving relevant code with a separate encoding model where the retrieved snippet serves as contextual reference for code completion. However, their retrieval scope is subject to a singular perspective defined by the encoding model, which largely overlooks the complexity and diversity inherent in code semantics.
To address this limitation, we propose ProCC, a code completion framework leveraging prompt engineering and the contextual multi-armed bandits algorithm to flexibly incorporate and adapt to multiple perspectives of code. ProCC first employs a prompt-based multi-retriever system which crafts prompt templates to elicit LLM knowledge to understand code semantics with multiple retrieval perspectives. Then, it adopts the adaptive retrieval selection algorithm to incorporate code similarity into the decision-making process to determine the most suitable retrieval perspective for the LLM to complete the code. Experimental results demonstrate that ProCC outperforms state-of-the-art code completion technique by 8.6\% on our collected open-source benchmark suite and 10.1\% on the private-domain benchmark suite collected from a billion-user e-commerce company in terms of Exact Match. ProCC also allows augmenting fine-tuned techniques in a plug-and-play manner, yielding 5.6\% improvement over our studied fine-tuned model.


==> sections/old_1_introduction.tex <==
\section{Introduction}

\begin{figure*}[h]
  \centering
  \includegraphics[width=0.95\linewidth]{figures/intro_case.pdf}
  \caption{Code completion scenarios demonstrating the contextual dependence of optimal retrievals. In Scenario 1, only Retriever 1 provides useful context. For Scenario 2,  Retriever 2 provides full list of relevant missing parameters. These cases underscore the need to retrieve multi-faceted interpretations and optimize selection based on semantic suitability. \colorbox{red}{\textcolor{black}{Red}} indicates the misleading information, \colorbox{green}{\textcolor{black}{Green}} represents the helpful hint.
  \yyy{unreadable figure}}
  \label{fig:intro-case}
\end{figure*}

Automated code completion aims at generating subsequent code tokens based on the ongoing incomplete code segments~\cite{convention_complete1, convention_complete2, convention_complete3, code_complete_Ngram, code_complete_attention, code_complete_rnn, code_complete_LSTM, lu2022reacc, zhang2023repocoder, knm}. Typically, it can significantly enhance the efficiency of software developers and reduce operating costs for corporations, e.g., averagely saving 3.65 keystrokes per completed token through browsing candidates recommended from automated code completion scheme~\cite{savekeystroke} \yyy{be more specific on the example. it seems quite general yet not reasonable}. Therefore, automated code completion has become widely incorporated into Integrated Development Environments (IDEs). For example, Microsoft's Pyright~\cite{pyright}, a static type-checking tool, powers the auto-completion feature for Python in VScode. 

Conventional automated code completion techniques generally rely on program analysis to generate syntax-conforming completions ~\cite{convention_complete1, convention_complete2, convention_complete3}, 
\thz{but cannot capture code semantics to generate line-level completions, which is expected by the developer \cite{code_expect}.}\yyy{so what?}. 
To alleviate such issues, many existing techniques~\cite{code_complete_Ngram, code_complete_attention, code_complete_rnn, code_complete_LSTM} adopt statistical or corpus-based techniques like N-Gram, Deep Neural Network~\cite{lecun2015deep} (DNN), Recurrent Neural Network~\cite{rumelhart1986learning} (RNN), and Long Short-Term Memory~\cite{hochreiter1997long} (LSTM) models to learn program semantics. However, they do not easily generalize across domains and require expensive data collection, annotation, and training efforts to adapt to new tasks, limiting their real-world applicability. 
% However, limited by the scale of the model and training data, these tools suffer from low prediction accuracy and are far from real deployment. 

Recently, by leveraging pre-training, large language models (LLMs) have been largely adopted on code and shown capable of varied tasks including code completion ~\cite{codet5+, starcoder, roziere2023codellama}. 
These models, trained on large code corpora \yyy{how large?}, can encode code knowledge and programming patterns into their large-scale parameters, remarkably outperforming the existing non-pre-trained techniques in both code understanding and generation tasks~\cite{zan2023large} in zero-shot settings.
% For instance, CodeT5+ ~\cite{codet5+} demonstrates strong gains over previous baselines in 10 tasks. 
For instance, Code LLaMA ~\cite{roziere2023codellama} is capable of completing 53.7\% of the text-to-code programming problems upon the HumanEval~\cite{chen2021evaluating} benchmark with no additional adaptation. However, when faced with complex logic or required to extrapolate beyond their training data, LLMs can struggle with incoherent or repetitive generations ~\cite{testcasedriven2021}. They may also hallucinate plausible but incorrect outputs ~\cite{llm_prob1, llm_prob2}. 
%\yyy{you do not mention fine-tune here. instead you directly go for rag. should introduce fine-tune is good but not enough and why to align with abstract.} \yyy{be more specific on introducing the mechanism of rag}
One potential solution to these issues is fine-tuning \yyy{[],}\yyy{i.e., ...}. However, fine-tuning LLMs, which typically consist of billions of parameters, proves to be a costly endeavor, both in terms of computational resources and time, making it impractical for many applications. For instance, fine-tuning the smallest LLaMA model typically requires a GPU workstation with 8 $\times$ \yyy{or $*$}A100 ~\cite{finetune_cost1, finetune_cost2}.
On the other hand, the Retrieval Augmented Generation~\cite{meta2020rag} (RAG) techniques offer a more feasible solution. Specifically, in a RAG model, given an input, related information is retrieved from a pre-defined knowledge source \yyy{a term?} and then used to guide the generation process. This retrieval process enables models to generate outputs that are coherent and relevant to the given context by grounding \yyy{make sure grounding is a correct usage} the generation in retrieved information. As a result, the RAG techniques effectively augment the understanding and generation capabilities of a model without the need for exhaustive fine-tuning. \yyy{make it clear here whether RAG techniques are SOTA.}
% To improve coherence, retrieval augmented generation (RAG) techniques ~\cite{meta2020rag} are proposed to enable LLM access to external memories or knowledge, as successfully applied in text generation ~\cite{li2022survey}. 
For instance, ReACC ~\cite{lu2022reacc} is the first work that integrates RAG for code completion, while RepoCoder ~\cite{zhang2023repocoder} introduces an iterative pipeline to enhance the retrieval process. KNM ~\cite{knm} builds an in-domain retrieval database and applies Bayesian inference for completion. 

Despite the promising results shown in the above-mentioned RAG-based techniques, they largely underestimate the importance of rich code semantics and informative program patterns. Moreover, they do not explore the selection of retrieved information. The optimal timing and content of retrieval remain unclear in the domain of code completion. 
\thz{
This ambiguity is exemplified in Figure~\ref{fig:intro-case}, which depicts three distinct scenarios and illustrates that different retrievals suit different completion contexts. In Scenario 1, Retriever 1 provides the hint "sslContext(SSLContext.getInstance())" which gives relevant context to help the generator complete the line. While Retriever 2 also hints "sslContext()", this is insufficient information to bridge the gap for completing the ``SSLContext.getDefault()''. Conversely, in Scenario 2, Retriever 2 presents the list of parameters that should be included in the function. This can be easily integrated by the generator to complete the return line, whereas Retriever 1 presents complex context and hinder the information delivery. These scenarios underscore the need to retrieve the code from multiple perspectives and select optimal retrievals tailored to the semantic context.
} \yyy{using a figure for an illustrative example in intro is overwhelming. Try a simpler one such that using a short text could be totally understandable. This figure could be moved to Section 2 and make it as ``Background and Motivation'' to motivate our approach.}

\yyy{looks like we do not highlight the need of prompt yet. }

Therefore, in this paper, we propose \ourmethod{} \yyy{make a better name}, a code completion framework which studies code semantics extensively and interpret code from multiple perspectives in order to dynamically select the information \yyy{what information?} based on the semantics \yyy{for what?}.
In particular, noticing that retrieving information from a single view has been shown insufficient to fully capture query semantics~\cite{multiquery3,multi-retri1}, \yyy{these are the discussion on the weakness of the previous approaches. should be included in the last paragraph. In this paragraph, we should only focus on the introduction of our approach.}
we adopt multi-retriever techniques~\cite{multi-retri2, multi-retri3} where multiple retrieval systems or algorithms are applied concurrently to provide larger coverage, diverse perspectives, and improved overall effectiveness to interpret code snippets from multiple viewpoints.
%In our approach for code completion, we are inspired by such multi-retriever techniques to interpret code snippets from multiple viewpoints. 
\thz{
We specifically examine two perspectives that are prominently used in RAG-based techniques, namely code context~\cite{lu2022reacc} and hypothetical line \cite{zhang2023repocoder}. Existing approaches construct code representations for retrieval either by encoding the code with auxiliary models—which requires additional efforts for training the encoding model—or by averaging the embeddings of the code, a process not inherently designed for representation. \yyy{still, the weakness should be included in the last paragraph.}
To minimize the extra cost associated with creating a new embedding model while preserving distinctive code representations, we employ prompt engineering to guide LLMs towards different viewpoints. \yyy{I imagine it would be better to highlight prompt engineering.} LLMs, trained to follow human preferences and instructions, can deeply understand semantics when prompted appropriately ~\cite{jiang-etal-2022-promptbert,jagerman2023query, Wang2023Query2docQE}. By harnessing LLM knowledge and crafting prompts towards targeting facets, we can expand code semantics from different lenses for more comprehensive retrieval. In particular, we craft the prompt, ``Embedding the following code snippets: [code]'' to encode the context of code, and the prompt, ``<PRE> [Prefix] <SUF> [Suffix] <MID>'' to generate the hypothetical line serving as its representation. Where the ``[code]'' refers to the unfinished code, ``[Prefix]'' and ``[Suffix]'' represents the code snippets before and after the target insertion point.
}
Furthermore, directly concatenating the retrieved information with input may confuse the generation of code, as illustrated in Figure~\ref{fig:intro-case}. To optimally select retrieved information, we employ contextual multi-armed bandit algorithms that make decisions conditioned on code semantics. By incorporating contextual information into the decision-making process, these algorithms adapt to the dynamic nature of code completion, handle uncertainty, and continuously improve through iterative learning. \yyy{the description here is still not quite technical.}

% TBD after experiments
To illustrate the generalizability of the proposed method, we instantiate \ourmethod{} on the State-Of-The-Art code completion model, \codellama{} and \starcoder{}, and extensively evaluate \ourmethod{} on various benchmarks [cite or explain]. The results of the experiment show that \ourmethod{} outperforms all previous RAG code completion methods. [later, more experiment findings]\yyy{simply introduce our benchmark. also introduce some representative experimental results}
% We further evaluate \ourmethod{} in industry practice. We deploy \ourmethod{} in an e-commerce company with around one billion Daily Active users (DAU). For initial deployment, we invited 1,000 programmers, representing various technology stacks. The results show that our method is good [to be discussed later].

% new discussion: multi-line code completion. Majority of previous work focus on single line completion. Copilot, Tabnine, CodeWhisperer all multi-lines. We're the first to evaluation multi-line. In this setting, we still need to compare single line completion. If no discussion on this, risk on being challenged why create new dataset, not using previous.


In summary, our contributions of this paper are listed as follows:
\begin{itemize}[leftmargin=*, topsep=0pt]
    \item We introduce \ourmethod{}, a novel retrieval augmented code completion framework based on multi-retriever and contextual bandits. \yyy{highlight prompt not bandits}
    In particular, we formulate the multi-retriever in a unified paradigm through
    prompting the LLMs, and actively choose the retrieval information based on contextual bandits. To our best knowledge, we are the first to introduce multi-retriever and contextual bandits for the code completion task.
    \item We conducted a thorough evaluation of code completion capabilities on open-source projects. Our findings demonstrate that \ourmethod{} yields a significant improvement in code completion capabilities compared to existing alternatives. \yyy{use some representative data}
    \item We demonstrate through ablation studies that \ourmethod{} provides a flexible framework to seamlessly integrate extra retrieval information to further improve code completion performance, which highlights the versatility of our method. \yyy{can we directly say that we are the first to show the different components adopted in our paper are advanced for enhancing the effectiveness of code completion}
    % \item \ourmethod{} has been rigorously evaluated within real enterprise environments. We sought and incorporated feedback from experienced developers, sharing invaluable insights that are crucial in the subsequent optimization for code completion domain.
\end{itemize}

==> tables/context_length.tex <==
% 这里是选择出来的381条长度超过8192的测试集即test-long的结果。
% \begin{table}[h]
% \centering
% \caption{Different context length 381 testsets}
% \begin{tabular}{cccccc}
% \hline
% \textbf{os} & \textbf{EM} & \textbf{ES} &\textbf{bandit} & \textbf{EM} & \textbf{ES} \\
% \hline
% 1k & 21.07 & 57.32 & 1k  & 40.25  & 70.03 \\ 
% 2k & 40.88 & 67.41 & 2k  & 42.45  & 72.89 \\
% 3k & 44.65 & 67.71 & 3k  & 51.89  & 75.70 \\
% 4k & 44.97 & 68.52 & 4k  & 49.06  & 73.89 \\
% 5k & 46.23 & 68.34 & 5k  & 43.4   & 68.40 \\
% 6k & 38.05 & 63.03 & 6k  & 42.12  & 68.50 \\
% 7k & 44.97 & 67.28 & 7k  & 53.14  & 75.05 \\
% 8k & 46.54 & 68.10 & 8k  & 37.74  & 65.76 \\
% \hline
% \end{tabular}
% \label{table:context_length}
% \end{table}


\begin{table}[h]
\centering
\caption{Different context length All testsets}
\begin{tabular}{ccccccc}
\hline
\textbf{os} & \textbf{EM} & \textbf{ES} &\textbf{\ourmethod{}} & \textbf{EM} & \textbf{ES} & \textbf{Time}\\
\hline
1k & 40.02 & 65.85 & 1k  & 44.57 & 68.30 & 0.1070s \\ 
2k & 45.61 & 70.54 & 2k  & 49.75 & 72.66 & 0.1217s \\
3k & 46.77 & 71.56 & 3k  & 51.76 & 74.23 & 0.1588s \\
4k & 47.90 & 73.12 & 4k  & 54.66 & 75.85 & 0.1842s \\
5k & 48.37 & 73.43 & 5k  & 54.73 & 76.16 & 0.2144s \\
6k & 47.90 & 73.21 & 6k  & 54.10 & 76.10 & 0.2533s \\

% 5k & 48.62 & 73.53 & 5k  & 51.59 & 74.59 & 0.1544s \\
% 6k & 47.80 & 73.31 & 6k  & 51.30 & 74.71 & 0.1833s \\
% 7k & 48.62 & 73.81 & 7k  & 52.61 & 75.56 & 0.1707s \\
% 8k & 48.85 & 74.04 & 8k  & 51.30 & 74.74 & 0.1740s \\
\hline
\end{tabular}
\label{table:context_length}
\end{table}


==> tables/database_chunk.tex <==
\begin{table}[h]
\centering
\caption{Database chunk}
\begin{adjustbox}{width=0.6\columnwidth}
\begin{tabular}{lcc}
\hline
\textbf{Method} & \textbf{EM} & \textbf{ES} \\
\hline
chunk30-overlap0 & 50.77  & 74.04 \\
chunk30-overlap15 & 52.14  & 75.07 \\
chunk30-overlap29 & 53.25  & 75.19 \\
chunk60-overlap0 & 0.195  & 0.3579 \\
chunk60-overlap30 & 0.195  & 0.3579 \\
chunk60-overlap59 & 0.195  & 0.3579 \\
\hline
\end{tabular}
\label{table:retrieval_selection}
\end{adjustbox}
\end{table}

==> tables/finetuning.tex <==
\begin{table}[h]
\centering
\caption{Compare with Fine-Tuning}
\begin{tabular}{lcc}
\hline
\textbf{Model} & \textbf{EM} & \textbf{ES} \\
\hline
Code Llama                     & 47.90  & 73.12 \\
Code Llama + FT                & 60.75  & 85.23 \\
Code Llama + \ourmethod{}      & 54.66  & 75.85 \\
Code Llama + FT + \ourmethod{} & 64.17  & 90.85 \\
\hline
% StarCoder & 45.04 & 70.50 \\
% StarCoder + FT & 57.87 & 84.70 \\
% StarCoder + \ourmethod{} & - & - \\
% StarCoder + FT + RAG & - & - \\
% \hline
\end{tabular}

\label{table:compare_with_fine_tuning}
\end{table}


==> tables/number_retrieval.tex <==
\begin{table}[ht]
    \centering
    \caption{Comparison of different retrieval numbers.}
    \begin{tabular}{lcccccc}
    \hline
    \multirow{2}{*}{\textbf{top-k}} & \multicolumn{3}{c}{\textbf{EM}} & \multicolumn{3}{c}{\textbf{ES}} \\
    \cline{2-7}
     & \textbf{FB.} & \textbf{RL.} & \textbf{ALL} & \textbf{FB.} & \textbf{RL.} & \textbf{ALL} \\
    \hline
    \textbf{Code Llama} & 34.97 & 68.91 & 47.90 & 64.49 & 87.15 & 73.12 \\
    \textbf{+top-1}  	& 41.16 & 76.58 & 54.66 & 67.22 & 89.86 & 75.85 \\
    \textbf{+top-2} 	& 41.82 & 76.77 & 55.14 & 67.75 & 89.93 & 76.20 \\
    \hline
    \textbf{+top-3} 	& 41.03 & 75.87 & 54.31 & 67.01 & 88.88 & 75.34 \\
    \textbf{+top-4} 	& 40.05 & 74.53 & 53.20 & 66.36 & 87.93 & 74.60 \\
    \textbf{+top-5} 	& 39.72 & 74.30 & 52.90 & 65.73 & 87.71 & 74.11 \\
    \hline
    % \textbf{StarCoder} & 30.78 & 67.96 & 45.04 & 60.42 & 86.72 & 70.5 \\
    % \textbf{+ top-1} & 30.64 & 69.55 & 45.46 & 59.28 & 87.1 & 69.94 \\
    % \textbf{+ top-2} & 29.32 & 68.79 & 44.45 & 57.62 & 86.77 & 68.79 \\
    % \textbf{+ top-3} & 29.46 & 68.94 & 44.6 & 57.37 & 87 & 68.73 \\
    % \hline
    \end{tabular}
    
    \label{table:number_retrieval}
\end{table}

% \begin{table}[ht]
%     \centering
%     \caption{Comparison of EM and ES scores for Code Llama model.}
%     \begin{tabular}{lcc}
%     \hline
%     \textbf{top-k}         & \textbf{EM} & \textbf{ES}\\
%     \hline
%     \textbf{\codellama{}}  & 47.90       & 73.12 \\
%     \textbf{+top-1}  	   & 54.66       & 75.85 \\
%     \textbf{+top-2} 	   & 55.14       & 76.20 \\
%     \hline
%     \textbf{+top-3} 	   & 54.31       & 75.34 \\
%     \textbf{+top-4} 	   & 53.20       & 74.60 \\
%     \textbf{+top-5} 	   & 52.90       & 74.11 \\
%     \hline
%     % \textbf{StarCoder} & 45.04 & 70.5 \\
%     % \textbf{+ top-1}   & 45.46 & 69.94 \\
%     % \textbf{+ top-2}   & 44.45 & 68.79 \\
%     % \textbf{+ top-3}   & 44.60 & 68.73 \\
%     % \hline
%     \end{tabular}
    
%     \label{table:number_retrieval}
% \end{table}
    

==> tables/rq1.tex <==
\begin{table}[h]
\centering
\caption{Fine-Tuning results}
\begin{tabular}{lcc}
\hline
\textbf{Models} & \textbf{EM} & \textbf{ES} \\
\hline
StarCoder-OS & 22.8 & - \\
StarCoder-Pretrain & 27.8 & - \\
StarCoder-SFT & 34.2 & - \\
\hline
Code Llama-OS & 23.6 & - \\
Code Llama-Pretrain & 29.9 & - \\
Code Llama-SFT & 36.5 & - \\
\hline
\end{tabular}
\label{table:fine_tuning_results}
\end{table}


==> tables/rq3.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
& 2023/11/13 & 2023/11/14 & 2023/11/15 & 2023/11/16 & 2023/11/17 & 2023/11/20 & 2023/11/21 & 2023/11/22 & 2023/11/23 & 2023/11/24 \\ \hline
OS & 10.53\% & 10.87\% & 10.64\% & 10.52\% & 10.28\% & 10.73\% & 10.31\% & 11.22\% & 11.36\% & 10.20\% \\ \hline
OS + gte-large & 11.67\% & 12.72\% & 10.78\% & 10.70\% & 10.32\% & 12.39\% & 11.87\% & 12.96\% & 13.32\% & 11.80\% \\ \hline
OS + BM25 & 11.79\% & 13.36\% & 10.93\% & 11.64\% & 10.84\% & 12.81\% & 12.13\% & 13.73\% & 13.78\% & 12.37\% \\ \hline
OS + Bandit & 13.01\% & 14.59\% & 12.81\% & 13.01\% & 11.56\% & 13.68\% & 13.53\% & 13.85\% & 15.11\% & 13.71\% \\ \hline
Pilot & 20.87\% & 21.31\% & 20.43\% & 20.01\% & 21.74\% & 20.00\% & 20.64\% & 21.14\% & 19.70\% & 22.88\% \\ \hline
\end{tabular}
\caption{Descriptive caption for the table.}
\label{tab:my_label}
\end{table}
